VindiCo: Privacy Safeguard Against Adaptation Based Spyware in Human-in-the-Loop IoT

Personalized IoT adapts their behavior based on contextual information, such as user behavior and location. Unfortunately, the fact that personalized IoT adapts to user context opens a side-channel that leaks private information about the user. To that end, we start by studying the extent to which a malicious eavesdropper can monitor the actions taken by an IoT system and extract users' private information. In particular, we show two concrete instantiations (in the context of mobile phones and smart homes) of a new category of spyware which we refer to as Context-Aware Adaptation Based Spyware (SpyCon). Experimental evaluations show that the developed SpyCon can predict users' daily behavior with an accuracy of 90.3%. The rest of this paper is devoted to introducing VindiCo, a software mechanism designed to detect and mitigate possible SpyCon. Being new spyware with no known prior signature or behavior, traditional spyware detection that is based on code signature or app behavior is not adequate to detect SpyCon. Therefore, VindiCo proposes a novel information-based detection engine along with several mitigation techniques to restrain the ability of the detected SpyCon to extract private information. By having general detection and mitigation engines, VindiCo is agnostic to the inference algorithm used by SpyCon. Our results show that VindiCo reduces the ability of SpyCon to infer user context from 90.3% to the baseline accuracy (accuracy based on random guesses) with negligible execution overhead.

==> abstract.tex <==
\begin{abstract}
Context-aware applications adapt their behavior based on contextual information, such as user behavior and location. Unfortunately, the fact that context-aware apps adapt to user context opens a side-channel that leaks private information about the user.
%Context-aware computing is a mobile computing paradigm in which applications can adapt their behavior based on contextual information, such as user behavior, location, and activity. Unfortunately, the fact that context-aware apps adapt to user context can open a side-channel that leaks private information about the user.
To that end, we start by studying the extent to which a malicious app can monitor the adaptations triggered by authentic context-aware apps and extract user's information.
In particular, we show a concrete instantiation of a new category of spyware apps which we refer to as \textbf{Context-Aware Adaptation Based Spyware (\spyware)}. Experimental evaluations show that the developed \spyware can predict users' daily behavior with an accuracy of $90.3\%$. %information about user's daily behavior. 
The rest of this paper is devoted to introducing \textbf{\sysname \footnote{Vindico is a latin word which means defend, protect, and punish.}}, a software mechanism designed to detect and mitigate possible \spyware apps.  Being a new spyware with no known prior signature or behavior, traditional spyware detection that is based on code signature or app behavior are not adequate to detect \spyware. Therefore, \sysname proposes a novel information-based detection technique. Moreover, \sysname applies several mitigation techniques to restrain the ability of the detected \spyware to extract private information. By having a general detection and mitigation engines, \sysname is agnostic to the inference algorithm used by \spyware.
\sysname is implemented as part of the Android system layer and evaluated using several case studies. Our results show that \sysname reduces the ability of \spyware to detect user context from $90.3\%$ to the baseline accuracy (accuracy based on random guesses) with negligible execution overhead. %to $43\%$ 
\end{abstract}

==> analysis.tex <==
%
%\begin{table*}[!t]
%\begin{tabular}{| L{3cm} | L{3cm} | L{1.5cm} | L{1.5cm} | L{1.5cm} | L{5cm} | }
%\hline 
%  & \multicolumn{4}{c|}{CPU Time (ms)} & Details \\ \hline \hline
%  &  & 2 adapt & 3 adapt & 4 adapt &  \\ \hline
%Parsing registry file & &$3.186$  &  $3.186$  & $3.187$  & Overhead on the loading time of the application \\ \hline
%
%Registry file processing & &$1.48$ & $2.22$ & $2.96$  & Constructing the necessary data structure. Overhead on the loading time of the application \\ \hline
%
%\multirow{4}{*}{\parbox[c]{3cm}{Tracking the values and filling the registry map at run time}} & total  & 0.066  &  0.076 &  0.076 &  \multirow{3}{*}{\parbox[c]{5cm}{Happens whenever an action is taken by the authentic context-aware application} }\\ \cline{2-5}
%																	      & Update current action value and get the last values of associated actions & 0.023 & 0.023 & 0.023 & \\  \cline{2-5}
%																	      & get corresponding context & 0.04 & 0.05 & 0.05 & \\  \cline{2-5}
%																	      & compute mutual information & 0.003 & 0.003 & 0.0035 &  \\  \hline
%
%Tracking API in monitor list and extract the corresponding mutual information&  &$0.056 $ & $0.090  $  &0.095 & {\parbox[t]{5cm}{Happens when a ``get'' API is called from one of the monitor list}} \\ \hline
%
%\end{tabular}
%\label{tbl:timinganalysis}
%\caption{Timing analysis of \sysname registry file processing and detection engine. Each module runs in a separate thread independently of the call of the API. The numbers are for registry files which have two adaptation tags, three adaptation tags, and four adaptation tags as described in Section~\ref{sec:registery} }
%\end{table*}
%
%

\begin{table}[!t]
\begin{tabular}{| c | c | c | c | }
\hline 
  & \multicolumn{3}{c|}{CPU Time (ms)} \\ \cline{2-4}
  & 2 adapt & 3 adapt & 4 adapt \\ \hline \hline
Parsing registry file & $3.186$  &  $3.186$  & $3.187$ \\ \hline

Registry file processing &$1.48$ & $2.22$ & $2.96$ \\ \hline

Overhead on a CA app & 0.066  &  0.076 &  0.076 \\ \hline

Overhead on other apps &$0.056 $ & $0.090  $  &0.095 \\ \hline

\end{tabular}
\label{tbl:timinganalysis}
\caption{Timing analysis of \sysname against increasing complexity of context-aware (CA) apps measured by number of adapt tags in the registry file.}
\end{table}



%\b{User study is carried over a Nexus 5 phone running a modified system image 
%for platform 5.0.1 API 22 ~\cite{aosp}. The execution time is obtained using the Android SDK tracer  ~\cite{trace}. 
%The size of the original system image for Android 5.1 is  $307$ MB, the modified system image that support  \sysname is $351$ MB. Hence, the overhead in the system image is $ 14\%$. \\
%}



We evaluate the timing performance of \sysname on Nexus 5 phones by running a modified system image for platform 5.0.1 API 22~\cite{aosp}. The execution time is obtained using Android SDK tracer. In order to reduce the performance overhead of \sysname on each API call, the Detection Engine is running in parallel thread. On the other hand, the Mitigation Engine runs on the same thread of any possible \spyware app.
%Hence whenever a set API is called as shown in Figure~\ref{fig:detectengine}, the call for the \sysname registry file processing and detection modules run independently to the call of the API. 
Table~\ref{tbl:timinganalysis} shows the CPU execution time when the complexity of the authentic context-aware app increases (reflected by the number of adapt tags in the registry file). As shown in Table~\ref{tbl:timinganalysis}, parsing and processing the registry file consumes approximately $6$ ms. Fortunately, this overhead takes place only during the installation of new packages to the phone. At run time, as shown in Table~\ref{tbl:timinganalysis}, \sysname adds negligible overhead (less than $0.1$ ms) thanks to the implemented data structures.
%
%for the mitigation engine, adding noise or mask the value returned by the API (as described in Section~\ref{sec:mitigation}) has negligible overhead. The reason for that is when a ``get API'' is called a flag is checked whether the caller application is marked as a \spyware or not. If yes, then the necessary mitigation policy takes place as in Section~\ref{sec:mitigation}. 
%Checking the flag and adding noise or masking the value returned have a negligible effect on the ``get API'' call. 
%
Finally, \sysname adds $44$ MByte to the original Android 5.1 system image resulting into an image of size  $351$ MByte.
 





==> detection.tex <==
\section{Detection Engine}\label{sec:detectionengine}
Malware detection techniques are traditionally based on a \emph{prior knowledge} of either the code signature or the behavior of \emph{similar} applications that are previously marked as spyware. However, as we showed in Section~\ref{sec:spycon_app}, existing signature-based detection mechanisms are not able to detect the developed context-aware spyware. Similarly, behavior-based detection techniques are not suitable to detect such spyware since no prior behavior is known to such spyware apps. Exacerbating the situation,  the behavior of a context-aware spyware is coupled to the behavior of the authentic context-aware apps. That is, if the authentic context-aware app triggers actions more frequently, the spyware will monitor the actions by calling the getter values APIs for these actions more frequently and so on. This behavior coupling hinders the usability of the behavior-based detection techniques.

In this section, we start by presenting a novel information-based detection engine that is 
agnostic to the spyware signature and behavior. In the second part of this section, we give details of how the proposed information-based detection is implemented in \sysname.

\subsection{Information-Based Detection}
The idea behind the information-based detection is to keep track of the ability of a spyware to infer phone context through monitoring actions triggered by this context. Recall that we do not have any prior knowledge or assumption on how a spyware performs its inference. To this end, we draw on information theory literature and, in particular, the notion of \emph{mutual information}. The mutual information quantifies the amount of correlation (or dependence) between two random variables. In particular, we are interested in continuously monitoring the mutual information between context and actions available to spyware. This mutual information measures---from the spyware point of view---the increase in certainty about context whenever actions are observed. This mutual information indicates the bound on the inference capability  of \emph{any} learning algorithm. Push into one extreme, if the mutual information is zero, then \emph{no} algorithm can infer context from monitored actions. In general, the lower the mutual information between context and actions, the lower the accuracy \emph{any} inference algorithm can get.

Based on this intuition, our detection engine keeps track of what actions have been monitored by each app, calculates an estimate of mutual information between the actual context and those actions monitored by this app, and assigns a  \emph{suspicion score} accordingly. This score is then passed to our Mitigation Engine (Section ~\ref{sec:mitigation}) as an indicator of magnitude of countermeasures, which aim for reducing amount of information possessed by suspicious apps.


To facilitate keeping track of mutual information between different contexts and monitored actions, we split the information-based detection engine into the following steps:~\\~\\
\textbf{- Step 1: Tracking Context-Aware App Behavior:} this step is carried over by recording all the actions taken by context-aware apps along with the contexts that triggered those actions.~\\~\\
\textbf{- Step 2: Computing Mutual Information:} In this step,  we use the time series stored in the previous step to calculate the mutual information between actions and contexts using standard algorithms for computing mutual information. Since we do not know a priori which actions is going to be used by a spyware aware to perform its adversarial inference, we compute the mutual information between the contexts and all different combination of actions associated with this context. ~\\~\\
\textbf{- Step 3: Monitoring Suspicious App Behavior: } Once an app invokes an API call that can be used to monitor an action, \sysname starts to suspect this app. This is done by  assigning a set of \emph{suspicious scores} for this app. These  \emph{suspicious scores} are equal to the mutual information between the action the app just monitored and all the contexts that may have triggered that action.

\b{Specific implementation details of the proposed information-based detection mechanism on Android platform is given in Section~\ref{sec:implementation}}

\subsection{False positives and false negatives - \g{This section needs revision for suspicious score we put on spyware and how we update after mitigation!}}
\r{In general, it's very hard follow the text in this subsection...}
Although mutual information is agnostic to the \r{actual behaviors (what behaviors?)} and/or inference algorithms used by the \spyware, some challenges need to be carefully addressed. \r{Arguably}, the most important issue is related to the convergence of estimating the actual mutual information from the data samples accessed by \sysname. That is, it is well known that calculating an estimate of mutual information with enough precision requires the access to multiple samples from both contexts and triggered actions \footnote{An estimate of the mutual information converges to actual mutual information asymptotically.}. \r{Hence, one can argue that a malicious spyware---who is aware of the existence of \sysname---may be tempted to reduce the frequency for which it monitors the actions with the goal of decreasing the number of samples used to estimate his mutual information and hence \emph{deceive} \sysname by reducing the associated \emph{suspicion score}. (Bo: The cause-effect is very weird for me)} In order to avoid such situation, we associate mutual information to actions instead of apps. That is, whenever an action takes place, we update the amount of mutual information between this particular action and all the context associated with it.  At any time point, once an app monitors this action, we copy the mutual information associated with this action to the app. Therefore, regardless of how frequent an app monitors actions, we associate to it the mutual information based on all samples in history not only on those he has access to.  
\v{That being said, false negatives (not assigning a suspicious score to a real \spyware) are not possible in our design because we keep track of all the apps that monitor the actions of context-aware apps. However, false positives (assigning a suspicious score to a non malicious app) are possible but because our mitigation engine is adaptive to the value of MI then if a small mitigation can decrease the MI with a very small amount of a false positive SpyCon and accordingly the false positives are not affected dramatically. Additionally, the main idea of detection here is to detect whether an application can have side channel information about another application whether it uses this information maliciously or not.}
The implementation details of the proposed information-based detection are given in the implementation details Section~\ref{sec:implementation}.




==> discussion.tex <==
\section{Discussion} \label{sec:discussion}



%\subsection{Knowing the installed applications}
%\sysname assumes that \spyware is effective if it knows what applications are already installed on the phone. %For the example we gave in Section~\ref{sec:spycon}, we assume that \spyware can know if a phone configuration app---that changes the phone settings based on the current location---is installed. %Hence, by monitoring the adaptation that happens in the phone settings, \spyware can detect the user's behavior. 
%The information about getting the installed apps can be retrieved from the Android API \texttt{GetInstalledApplications()}. While one can argue that by protecting this API in the manifest file, we can protect against any \spyware. However, this information can still be retrieved by running a shell command inside \spyware using \texttt{getRuntime().exec()} and listing the \emph{data directory} which contains the names of the applications installed on the device. One of the possible incentives of why Android may allow the use of \texttt{exec()} method (though it has this security hole of knowing what are the running apps/installed apps/foreground and background apps~\cite{zhou2013identity}) is to allow augmenting functionality. For example, one can execute a shell script which can be a lot shorter than Java code.  
%\b{Even if we assume that Android protects this API by adding a permission for using it, the user will not relate that this API can be used in the side channel attack exploited by the purposed \spyware.}


%to do the same amount of work. %One other benefit of having \texttt{exec()} method is 
%\b{Another benefit is to do dynamic library linking for 3rd party application which may exceed the allowable size of included APK files, and one way to link it through runtime is to use \texttt{exec()} method. }

%Unlike Android platform, iOS does not allow to ``explore'' what are the running apps. However, there was a way to do that, since apps can register an URL to respond external messages, one can use URL to check whether a particular app is on the device, one famous project is called iHasApp~\cite{ihasapp}. However, it was also broken in 2011 since Apple deprecates \emph{canOpenURL} method. Hence, though one can issue a request and pass the task to the second app, the app will never be informed the app is existed or even opened.

%\subsection{Collaborative \spyware} \vspace{-1mm}
Several apps can cooperate with each other by collecting partial information and aggregate it to infer the user's behavior. One work that tries to reduce the aggregation of app usage behavior is LinkDroid~\cite{linkdroid}. LinkDroid measures the underlying linkability across apps and informs the end users of the possible risks. \sysname detection engine can indeed be augmented with tools like LinkDroid to detect if there are collaborative apps to have a collective suspicion score across all of these apps.



%\subsection{Beyond phone settings\r{remove this section}}\vspace{-1mm}
%summarize Mostafa's survey on this \url{https://docs.google.com/document/d/12LPUIQ5ILFP4wlkZeUEBr3V4qnhOReoAwQgsIQocFY4/edit}
%The \spyware example shown in Section~\ref{sec:spycon} focused on the phone settings % and their corresponding APIs
% listed in Table~\ref{tab:phonesettings} to leak sensitive information. In order to know the actual usage of these APIs in applications presented in the market and hence estimate the significance of \spyware, we performed static analysis on the the top 100 downloaded apps from the Google Play store. Our analysis shows that some of the APIs that are used by the proposed \spyware are widely used across these applications. In particular, our study shows that 83\% of the apps checks whether WiFi is turned on using the same API used by the proposed phone-setting \spyware. Similarly, 80\% of the apps get the current audio volume %and 75\% read the MAC address of the current WiFi access point both using the same APIs used by the proposed phone-setting \spyware.
%  The results of the overall analysis are shown in Figure~\ref{fig:api_usage}.
%\begin{figure}[!h]
%\centering 
%\includegraphics[trim={0 0.1cm 0 0.1cm},clip,width=0.5\textwidth]{tikzfigure/common_get_data.pdf}
%\caption{The percentage of applications from 100 downloaded free Android apps that make use of the APIs mentioned in Table~\ref{tab:phonesettings}.\vspace{-3mm}}
%\label{fig:api_usage}
%\end{figure}
%\begin{figure}[!h]
%\centering
%\includegraphics[trim={0 0.1cm 0 0.4cm},clip,scale=0.5]{figures/get_ccdf2.eps}
%\caption{CCDF of number of \emph{get} phone settings APIs used by the top 100 downloaded applications.\vspace{-4mm}}
%\label{fig:api_ccdf}
%\end{figure}
%We also notice that most of those applications  use more than one API to get the values of the settings in Table~\ref{tab:phonesettings}. 
%The complementary cumulative distribution function (CCDF) curve shown in Figure~\ref{fig:api_ccdf} for the number of used APIs per application indicates that around 60\% of the sampled applications use $4$ or more APIs listed in Table~\ref{tab:phonesettings}, which are the functions considered by our exemplar \spyware.

 %The popularity of these APIs among applications indicates how impractical it is to identify \spyware apps by simply enumerating how many phone settings or similar APIs they use. Obviously, this naive approach will lead to many false positives. Therefore, a more clever detection approach such as the information-based detection engine we discussed in Section~\ref{sec:detectionengine} is required.

%% This what was written in this section
%While the study in Section~\ref{sec:sca} shows that the proposed \spyware is practical,  \spyware is not limited only to the phone settings listed in Table~\ref{tab:phonesettings}. In general, \spyware can take advantage of any pair of  \texttt{get} and \texttt{set} methods. More specifically, Android framework APIs has many examples of this kind of get-set pairs existing in \texttt{PackageManager}, \texttt{ClipboardManager}, and others.
\vspace{-1mm}


%False negatives (mistakenly not assigning a suspicion score to a real \spyware) are \r{highly unlikely (or impossible).}  
%However, false positives (mistakenly assigning a suspicious score to a non-malicious app) are indeed possible. These false positives occur because the information-based detection engine searches for apps that have side channel information about other apps whether they use this information maliciously or not. \r{Accordingly, this will affect the utility of the benign application. To tackle this problem in our system, \b{(to harness such drawback,)} a higher level logic, e.g. informing the user, may be used. Since we are showing a new kind of spyware, we mark these apps as undetected spyware and inform the user. If the user decides that the app is not malicious, then our system will let it behave normally. The \textbf{privacy-utility tradeoff problem} or sometimes called \textbf{risk-value tradeoff problem} has been addressed in previous work~\cite{chakraborty2013protecting, pipes2014multitiered}. Indeed our Mitigation Engine can be augmented by one of the previously proposed solutions for this problem.} \vspace{-2.5mm}

%However, we note that (1) mitigation engine is adaptive in nature to the value of mutual information. That is if a small mitigation action can decrease the mutual information 
%
%
%with a very small amount of a false positive SpyCon and accordingly the false positives are not affected dramatically. Additionally, the main idea of detection here is to detect whether an application can have side channel information about another application whether it uses this information maliciously or not.




==> implementation.tex <==
%\begin{figure}[t]
%  \centering
%    \includegraphics[width=\columnwidth, trim={1cm 2.5cm 0.5cm 0.2cm},clip]{figures/architecturekeynote3}
%     \caption{\sysname architecture. Context-aware application is registered in \sysname by context-adaptation registration module. The behavior of the context-aware app is monitored, and a possible \spyware is detected by the Detection Engine, then the adequate mitigation technique is taken by the Mitigation Engine.%\sysname service runs in the system space while its app interface (\sysname manager) runs in the user space. %Context-aware application is registered in \sysname by context-adaptation registration module. The behavior of the context-aware app is monitored and a possible \spyware is detected by the Detection Engine, then the adequate mitigation technique is taken by the Mitigation Engine.
%     \vspace{-5mm}}
%     \label{fig:androidarch}    
%\end{figure}

%\begin{figure*}[!th]
%\centering
%\includegraphics[width=0.86\textwidth, trim={0 16cm 0 0},clip]{figures/registryfileprocessing_r3}
%  \caption{Context-adaptation registration. At installation time, \sysname checks the existence of a registry file and starts processing it accordingly. Registry file processing constructs all necessary data structures that are needed  by the detection and mitigation engines.\vspace{-4mm}}\label{fig:registryfileprocess}
%\end{figure*}


%\begin{figure*}
%  \begin{minipage}[c]{0.67\textwidth}
%    \includegraphics[trim={0 17.5cm 10.4cm 0},clip, width=0.5\textwidth ]{./figures/detectionengine_r5}
%  \end{minipage}\hfill
%  \begin{minipage}[c]{0.3\textwidth}
%    \caption{
%       \sysname Detection Engine. 
% When a context-aware app calls a \emph{setter} API to adapt to user context, \sysname Service intercepts the call and checks if this API call is 
%  in the \emph{Adaptation Record}. Next, the mutual information algorithm updates the corresponding Mutual Information Table based on the new data recorded in the Adaptation Record.  Whenever an app calls a \emph{getter} API that matches one of the API in the \emph{Protection Lists}, the mutual information corresponding to the \emph{getter} API is retrieved and assigned to this app as a suspicion score. 
%}  \label{fig:detectengine}
%  \end{minipage}
%\vspace{-4.5mm}  
%\end{figure*}
%
\vspace{-0.2cm}
\section{
Implementation}\label{sec:implementation} 
We extended the Android system layer to add the three main parts of  \sysname as shown in Figure~\ref{fig:androidarch}. 
%as explained in Section~\ref{sec:sysarch}. The three main parts of \sysname (context-adaptation registration, detection engine, and mitigation engine) %are implemented in the Android system layer 
In this section, we explain the  implementation details of all the three modules.
%\o{(Bo: Are we going to put percentage here?)}

\vspace{-0.1cm}
\subsection{\sysname Context-adaptation Registration}\label{sec:regImpl}
%As mentioned in Section~\ref{sec:contadaptreg}, the context-action relationships have to be learned so that \sysname can track how likely a \spyware can infer user's context. 
In this section, we explain, with an example in Figure~\ref{fig:registryfileprocess}, the data structures used by \sysname to track the information possessed by possible \spyware apps.

%how \sysname tracks the ability of \spyware in terms of infer user's context. We achieve this by implementing the following data structures.% that are needed to track this relation.  



%\subsubsection{\textbf{Registry file processing}}\label{sec:registryprocess}\vspace{-1mm}
%%Whenever a new application is installed, \sysname checks the existence of a registry file. 
%Once \sysname finds a registry file, several post-processing steps will take place during the installation time for this context-aware application. In particular, \sysname parses the XML file, and the extracted information is then used to fill the following data structures:%\vspace{2mm} ~\\


%\textbf{- Adaptation Records}: The purpose of this data structure is to keep track of the actions taken by the authentic context-aware apps and the changes in the context that triggered such actions. An adaptation record data structure is created for each \emph{adaption} in the registry file. Upon changes in either context or actions, \sysname appends a record to these data structures consisting of both the context and the actions along with a timestamp.

%\textbf{- Protection Lists}: 
%In this data structure, we hold a list of all APIs that a~\spyware can use to monitor the actions that are triggered by the authentic context-aware apps.
%Take the registry file example in Figure~\ref{fig:registry_example_2}, two lists are constructed for the two adaptation tags. The first Protection List includes two functions, \texttt{getRingerMode()} and \texttt{getAlarmVolume()}. Similarly, the second list contains the corresponding getters of the three mentioned functions.





\vspace{-0.1cm}
\subsubsection{\textbf{Adaptation Record}} \label{sec:registrymap}
The purpose of this data structure is to keep track of the actions taken by the authentic context-aware apps and the changes in the context that triggered such actions. An adaptation record table is created for each \emph{adaptation} in the registry file. Upon changes in either context or actions, \sysname appends a record to these tables consisting of both the context and the actions along with a timestamp.
%
%The schema of the \emph{Adaptation Record} table is inflated by all the \emph{context} and the \emph{action} elements within each \emph{adaptation} tag declared in registry files. F
Figure~\ref{fig:registryfileprocess} demonstrates two adaptation record tables corresponding to two \emph{adaptation} tags.
%For example, the registry file  Figure~\ref{fig:registryfileprocess} is processed into two \emph{registry maps}.
Initially, these tables are empty and are filled as the context-aware app decides to perform a new adaptation. 
%Whenever an adaption %(i.e., context changes and corresponding actions)  is made, \sysname appends a record to the end of these tables. 
 These tables are then used by the \emph{Detection Engine} to estimate the amount of \emph{information} that can be potentially retrieved if some actions are monitored. %To facilitate the generation of the \emph{Adaptation Records}, the registry file processing module
% We use a predefined map that associates each API name with a unique identification number (ID) as shown in Figure~\ref{fig:registryfileprocess}.

\vspace{-0.1cm}
\subsubsection{\textbf{Protection Lists}}
Most of the setter APIs in the Android Framework managers have corresponding getter APIs, and a malicious app can use these getter APIs to monitor any change in actions triggered by authentic context-aware apps. For example, if an authentic context-aware app uses \texttt{setRingerMode()}, a \spyware can use \texttt{getRingerMode()} to track the action triggered by this authentic app.
%Since a \spyware can learn enough information from these getter APIs, we summon them into lists which are called \emph{Protection List}. %As shown in Figure~\ref{fig:registryfileprocess}, one Protection List corresponds to one \emph{adaption} tag in the registry file. %Each element in these lists represents a getter API coded by its ID.
\sysname summon all getter APIs (which can potentially leak user context) into a list called \emph{Protection List}. Take the registry file example in Figure~\ref{fig:registry_example_2}, the corresponding Protection Lists after parsing the registry file are shown in
Figure~\ref{fig:registryfileprocess}. In particular, two lists are constructed for the two adaptation tags. The first Protection List includes two functions, \texttt{getRingerMode()} and \texttt{getAlarmVolume()}. Similarly, the second list contains the corresponding getters of the three mentioned functions.
%Whenever a \spyware accesses any method in the Protection List, it is suspected by \sysname.
%There are two actions taken in the first adaptation tag, the first one is \texttt{setRingerMode()} with ID \texttt{$a_1$} thus we put its ID \texttt{$g_1$} to the first entry in the first Protection List.
%\o{(Bo: rephrase or delete) These Protection Lists are then being referenced by the Detection Engine.}% as explained in Section~\ref{sec:detectengineimpl}. 

\vspace{-0.1cm}
\subsubsection{\textbf{Mutual Information Tables}}\label{sec:mutualtables}
As explained in Section~\ref{sec:sysarch}, the Detection Engine depends on information-based technique. 
\sysname generates one \emph{Mutual Information Table} per \emph{adaptation} tag in the registry file. The table consists of the power set of all the actions, and each row stores the mutual information of the subset of the actions and the context. Figure~\ref{fig:registryfileprocess} gives two examples of Mutual Information Tables. All the entries are initialized to zeros and will be updated by the Detection Engine.

%To enable this detection mechanism, \emph{Mutual Information Tables} are generated by \sysname. Each table associates with one \texttt{adaptation} tag in the registry file. The rows of this table represent all possible subsets of the actions within an adaptation to capture all possible information that \spyware may obtain by monitoring any subset of these actions. Back to our example in Figure~\ref{fig:registryfileprocess}, two Mutual Information Tables are generated. Initially, these tables are empty and will be filled by the Detection Engine.

%To enable this detection mechanism, %upon the installation of an APK, the registry file is processed and 
%\emph{Mutual Information Tables} are generated by \sysname. Each table associates with one \texttt{adaptation} tag in the registry file. The rows of this table represent all possible subsets of the actions within an adaptation to capture all possible information that \spyware may obtain by monitoring any subset of these actions.
% 
% that is generated by the registry file processing module is designated to help the Detection Engine to create knowledge about how much information the malware has on the user's contexts by monitoring the changes in the set of actions. Hence, the data structures we designed for this are tables for mutual information between the values of contexts and the values of actions. 
% 
%By forming all the subsets of actions triggered by authentic apps, we capture all possible information that \spyware may obtain by monitoring any subset of these actions. 
%Back to our example in Figure~\ref{fig:registryfileprocess}, two Mutual Information Tables are generated. %each with three rows as the power sets of two actions (deducting the empty action set).
% Initially, these tables are empty and will be filled by the Detection Engine. %at runtime as explained in Section~\ref{sec:detectengineimpl}.

%Fortunately, the overhead of creating these data structures takes place only during the installation of new packages to the phone. We will show the timing overhead of parsing the registry file and creating these data structures in Section~\ref{sec:analysis}.
%\begin{figure*}[t]
%\centering
%\includegraphics[trim={0 18cm 0 0},clip,scale=0.2, width=0.86\textwidth , height=6.1cm]{./figures/detectionengine_r3}
%\caption{\sysname Detection Engine. %\sysname Manager intercepts the calls of \emph{setter} and \emph{getter} APIs.
% When a context-aware app calls a \emph{setter} API to adapt to user context, \sysname Manager intercepts the call and passes it to \sysname Service which in turn checks this API call %versus information stored
%  in the \emph{Adaptation Record}. Next, the mutual information algorithm updates the corresponding Mutual Information Table based on the new data recorded in the Adaptation Record.  Whenever an app calls a \emph{getter} API that matches one of the API in the Protection Lists, the mutual information corresponding to the \emph{getter} API is retrieved and assigned to this app as a suspicion score. Finally, the Mitigation Engine reads this suspicion score and apply adequate actions.
%\vspace{-4.5mm}}
%\label{fig:detectengine}
%\end{figure*}

\vspace{-0.1cm}
\subsection{\sysname Detection Engine}\label{sec:detectengineimpl}


%In particular, the information-based detection engine works as follows: ~\\
%\textbf{Step 1: Tracking Context-Aware App Behavior:} In this step, we use the adaption record data structures to record all the actions (taken by context-aware apps) along with those context causing these actions. ~\\
%\textbf{Step 2: Computing Mutual Information:} We compute the mutual information between the action and the context time series from the previous step. Since we do not know a priori which (set of) actions are going to be used by a \spyware for adversarial inferences, we compute and store the mutual information between the context and the power set of all actions.~\\% (the power set). %associated with this context.
%\textbf{Step 3: Monitoring Suspicious App Behavior:} Whenever an app invokes a getter API  that can be used to monitor an action, \sysname starts to suspect this app. In particular, \sysname assigns  a set of \emph{suspicion scores} to this app. Each element in these \emph{suspicion scores} corresponds to one protection list. The value of the suspicion score is equal to the mutual information derived from the actions monitored in the corresponding protection list.

%Implementation details of information-based detection mechanism in \sysname are given in Section~\ref{sec:detectengineimpl}.




The Detection Engine is a core module in \sysname that implements the information-based detection mechanism. %An illustrative figure of the full detection flow implementation is shown in Figure~\ref{fig:detectengine}.
 We provide the details of our implementation with an illustration of the detection flow in Figure~\ref{fig:detectengine}. %\vspace{-2mm}
 In particular, the information-based detection engine works as follows:
 
 \vspace{-0.1cm}
\subsubsection{\textbf{Step 1: Tracking Context-Aware App Behavior}}
The first step is to keep track of all the changes in context. Whenever a change occurs in a context, \sysname timestamp such change and record the timestamp along with all the actions (taken by context-aware apps) and the corresponding context that caused these actions. This step is performed through filling in these values in the \emph{Adaptation Record} table.
%discussed Section~\ref{sec:registrymap}. 
%This \emph{Adaptation Record} is nothing more than a table that keeps the history of the time series corresponding to changes in contexts and actions. 
%One possible implementation is to edit all the setter and getter APIs in the Android Framework managers in order to fill in the values in the Adaptation Record. Unfortunately, due the sandboxing mechanism implemented by Android, the Android Framework managers are part of the user space and hence Android instantiates multiple copies of the Android Framework  managers, one for each running app. On the other hand, the \emph{Adaptation Record} data structures needs to be stored in the operating system space since the information stored in them are going to be used to detect if other apps are malicious or not. 
%Therefore, 
%We split our implementation into two layers, a \sysname Manager and a \sysname Service (see Figure~\ref{fig:androidarch}). \sysname Manager is implemented as an extension of the Android Framework Manager and hence resides in the \emph{user space}. This layer monitors all the calls initiated by authentic context-aware apps and passing this information to the \sysname Service which is implemented in \emph{system space}. 

Note that we have a separate Adaptation Record for each map between context and actions. Therefore, even if a certain action may have been triggered by multiple changes in different context, we will treat each context separately, and all the corresponding Adaptation Record tables will be updated

%Once the
% \emph{Detection Engine} receives the information about the APIs called by the authentic app, it retrieves the corresponding values of the context and actions and updates the \emph{Adaptation Record} accordingly\footnote{\b{Recall that we map each context to the corresponding actions. Hence, even if the \emph{same} adaptation happened to \emph{multiple} contexts as in the example we gave in the registry file, each action-context map (Adaptation Record) will be treated separately.}}. 
 
\vspace{-0.1cm}
\subsubsection{\textbf{Step 2: Computing Mutual Information}}
The next step is to calculate the mutual information based on the time series stored in the \emph{Adaptation Record} tables.  Since we do not know a priori which (set of) actions are going to be used by a \spyware for adversarial inferences, we compute and store the mutual information between the context and the power set (all different combination) of all actions.
%As we discussed in Section~\ref{sec:detection}, 
%we compute the mutual information between the context and all different combination of actions associated with this context. 
These values are then stored in the \emph{Mutual Information Tables} and are updated whenever new entries are added to the \emph{Adaptation Record}.
%
%The exemplar app shown in Figure~\ref{registryfileprocessing} changes the camera settings and Jpeg compression modes based on user transportation modality and phone battery level. For instance, when a user is running and the phone has sufficient battery level, the app sets the camera focus to ``continuous focus mode,'' the scene mode to ``action mode,'' and the Jpeg saving quality to the maximum value \footnote{These values are provided by Android APIs that the developer can use directly.}. At run time, the monitor engine keeps recording both contexts and action adaptions in the registry map (Section~\ref{sec:registrymap}). In this case, the monitor engine records these values in RegistryMap 2.  %and refreshes the map every day. %Our heuristic assumes that by recording the entries in the map per day is enough to know the relation between the change in the values of the set of context and the set of actions.
% In the rest of this section, we explain how we get this relation in order to quantify the effect of monitoring the set of actions in retrieving information on the context and detect any possible \spyware.   This is done by the three main functions of the detection module: 
%\begin{enumerate}
%\item It calculates the mutual information between the action values and the context values. 
%\item It uses all the ``monitor lists'' created by the registry file processing phase as explained in Section~\ref{sec:registery} in order to know which sets of actions the detection engine needs to monitor (Section~\ref{sec:detect1}).  
%\item It tracks any application that uses any APIs in any one of the ``monitor lists'' (Section~\ref{sec:detect2}).
%\item It outputs a mapping between ConMaN application name and a number associated with each ``monitor list''. This number is an indication of how much information this application has on the context associated with this ``monitor list''.  Since an application can monitor subsets of the actions in any ``monitor list'', the associated number with each monitor list is different from one application to another  (Section~\ref{sec:detect3}). 
%\end{enumerate}



\begin{figure*}[t]
%\floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=0.4\textwidth}}]{figure}[\FBwidth]
\centering
%\includegraphics[trim={0 18cm 0 0},clip,scale=0.2, width=0.86\textwidth , height=6.1cm]{./figures/detectionengine_r4}
{\includegraphics[trim={0 17.5cm 10.4cm 0},clip, width=0.86\textwidth ]{./figures/detectionengine_r5}
}
{\caption{\sysname Detection Engine. %\sysname Manager intercepts the calls of \emph{setter} and \emph{getter} APIs.
 When a context-aware app calls a \emph{setter} API to adapt to user context, \sysname Service intercepts the call and checks if this API call is %versus information stored
  in the \emph{Adaptation Record}. Next, the mutual information algorithm updates the corresponding Mutual Information Table based on the new data recorded in the Adaptation Record.  Whenever an app calls a \emph{getter} API that matches one of the API in the \emph{Protection Lists}, the mutual information corresponding to the \emph{getter} API is retrieved and assigned to this app as a suspicion score. \vspace{-0.4cm}%Finally, the Mitigation Engine reads this suspicion score and apply adequate actions.
}  \label{fig:detectengine}}

\end{figure*}


%\subsubsection{Step 2: Computing mutual information}
%We use mutual information \b{by applying .... algorithm}~\cite{} between the two time series provided in the ``registry map'' in order to estimate how much the information about the context ConMan can retrieve if it can monitor the values of the actions. \b{ The way this algorithm works is by doing the following steps:} \\
%\begin{enumerate}
%\item ..
%\item ...
%\item ....
%\end{enumerate}
%Hence, by the end of running this algorithm a value is returned that indicates the mutual information between the set of actions and the context. From the information theory point of view, If the returned value is high, then we can say that ConMan \emph{can} construct a smart machine learning kernel that we are agnostic about to infer the value of the context and vice versa.  The way ConMan constructs this machine learning kernel is out of the scope of this paper. However, to quantify how much ``high'' and ``small'' the returned values are we need to set threshold. Setting the threshold in the mutual information is not an easy task ~\cite{}. However, we will show next our heuristics in setting this threshold. 
%

%\subsection{Setting threshold}
%\r{This section needs to be revised to make sure that the technical information written is correct - Needs an information theory person to revise it} - Maybe Yasser .\\
%The importance of setting the threshold is to declare how much suspicious we are about ConMan if it monitors the set of actions in one of the ``monitor list''. Based on the this threshold, the mitigation technique will differ to hinder ConMan performance.  \\
%There are two problems in setting the threshold, the first one is that we do not assume any knowledge on the way ConMan is inferring the context. For example, in the case study we show in Section~\ref{sec:conman}, ConMan is not trying to get the actual GPS location but trying to infer daily behavior of the user which is a much easier than retrieving the actual GPS location. The second problem is that context that the monitor engine is recording can have continuous values like GPS location, accelerometer values, ... etc. but the \b{.... algorithm} works on discrete values. Hence, sampling these continuous values is needed with calculated resolution in order to get meaningful values returned after running the \b{.... algorithm}. We address these two problems as follows. 
%\\
%\subsubsection{First problem: labels are not known}
%We address the first problem by using the fact of \b{mutual information inequality - not sure of the term}~\cite{} which states that the information presented in a processed data is less than the information presented in the actual data.  
%\begin{equation}H(x, y) = I(x,y) - I(x)I(y)\end{equation}
%\begin{equation}H(x', y) = I(x',y) - I(x')I(y) \end{equation}
%\begin{equation} I(x,y) \geq I(x',y) \end{equation}
%\begin{equation}I(x') \overset{?}{\geq} I(x) \end{equation}
%\begin{equation}H(x,y) \overset{?}{\geq} H(x',y) \end{equation}
% 
% \b{write some sentences on how we address this problem based on the above equations by setting more aggressive threshold on the raw context which will in return restrict the threshold of the inferred context.  Explain what these equations actually mean.}\\
% 
% \subsubsection{Second problem: continuous values of the context}
% \b{We address the second problem by sampling the continuous data into  .... that are based on ... algorithm .... bla bla. Have no idea what to write here!}
 
 
% \begin{table*}[!t]
%\centering
%\begin{tabular}{c c c||c}
%
%\begin{tabular}{| L{1.5cm} | L{0.6cm} | }
%\hline 
%Monitor List 1  & MI  \\ \hline
%\hline
%$a_1$ & $x_1$ \\ \hline
%$a_1$, $a_2$ & $y_1$  \\ \hline
%$a_1$, $a_2$, $a_3$ & $z_1$  \\ \hline 
%$a_2$, $a_3$  & $w_1$ \\ \hline
%$\dots$ & $\dots$ \\ \hline
%\end{tabular}
%&
%\begin{tabular}{| L{1.5cm} | L{0.6cm} | }
%\hline 
%Monitor List 2 & MI  \\ \hline
%\hline
%$a_4$ & $x_2$ \\ \hline
%$a_4$, $a_6$ & $y_2$  \\ \hline
%$a_4$, $a_5$, $a_6$ & $z_2$  \\ \hline 
%$a_5$, $a_6$  & $w_2$ \\ \hline
%$\dots$ & $\dots$ \\ \hline
%\end{tabular}
%&
%$\dots$
%&
%\begin{tabular}{| L{2cm} | L{1.5cm} | L{1.5cm} | L{1.5cm} | L{1.5cm} |}
%\hline 
%Package Name & Monitor List 1 & Monitor List 2 & $\dots$ & Monitor List n \\ \hline
%\hline
%name 1 & $y_1$ & $x_2$ &  $\dots$ & $w_n$ \\ \hline
%name 2 & $x_1$ & $y_2$ &  $\dots$ & $z_n$ \\ \hline
%name 3 & $w_1$ & $z_1$ &  $\dots$ & $x_n$ \\ \hline
%$\dots$ 		   & $\dots$ & $\dots$ &  $\dots$ & $\dots$ \\ \hline
%\end{tabular}
%
%
%\end{tabular}
%\caption{\r{remove this table!}Mutual Information for each monitor list between the set of actions and the associated context. Each row represents one monitor list in \sysname system. The entries in each row are the mutual information between a subset of actions and the associated context with this monitor list. } \label{tbl:mutualinformation}
%\end{table*}
 
 
% 
% \subsection{Combination of all actions} \label{sec:allcombination}
% \b{In calculating the mutual information between set of actions and set of context, we must consider all the combination of the set of actions with the context. The reason is that an application can only read subset of actions from a monitor list and still has a high mutual information with the context. We need to have a relation between any subset of actions with the context in each monitor list.   When these numbers are calculated, they are saved per monitor list.  This is achieved by constructing \emph{mutual information map} associated with each monitor list. For each monitor list, each action item has an identification number and using permutation of these identification numbers, a mutual information value is reported. Hence, for the first monitor list example in Figure\ref{fig:monitorlist} which has 3 actions, the \emph{mutual information map} will have $2^3 - 1$ entries.  However, to create this for all possible combination for every monitor list, will be time consuming. } \r{talk about some heuristic used to reduce this time in practical }
%
%After calculating all the mutual information between all the subsets of actions  and the context for each monitor list in \sysname system. This information is recored that holds this information to be used later in the detection module (Section ~\ref{sec:detection}). 
\vspace{-0.1cm}
\subsubsection{\textbf{Step 3: Monitoring Suspicious App Behavior}}\label{sec:detect1}\label{sec:suspicious_score}
The last step is to use all the \emph{Protection Lists} to track the behavior of suspicious apps. %Recall that Protection Lists contain the IDs of the getter APIs a \spyware can monitor to reveal the context. Hence
%
Whenever an app invokes a \emph{getter} API that can be used to monitor an action (i.e., an API in the \emph{Protection List}), \sysname starts to suspect this app by assigning a \emph{suspicion score} to this app.
%\sysname assigns  a set of \emph{suspicion scores} to this app. Each element in these \emph{suspicion scores} corresponds to one protection list. The value of the suspicion score is equal to the mutual information derived from the actions monitored in the corresponding protection list.
%
% Any call from an app to any of the APIs in the \emph{Protection Lists} should raise the alarm that this app is a potential \spyware. %Thanks to the two-layered approach of \sysname (i.e., the \sysname Manager and \sysname Service layers), \sysname can track all the APIs' call. Therefore,
%  Once an app calls a \emph{getter} API marked in one of the \emph{Protection Lists}, 
%  \sysname assigns a \emph{suspicion score} to this app which 
  The value of this \emph{suspicion score} is
  equal to the mutual information associated with the \emph{getter} API (invoked by the app) which is stored in the \emph{mutual information tables}.
  %
Since the same app may have called several \emph{getter} APIs belonging to different \emph{Protection Lists}, \sysname associates a set of \emph{suspicion scores} (instead of just one \emph{suspicion score}), one per \emph{Protection List} in a table that is called \emph{applications suspicion scores} table (see Figure~\ref{fig:detectengine}). %These \emph{suspicion scores} are the input to the Mitigation Engine. %described in Section~\ref{sec:mitigationimpl}.

%To enhance the performance of the Detection Engine upon setter/getter APIs being called, \sysname forks a separate thread in order to monitor the values and update the corresponding data structures. We show the overhead in the Detection Engine in Section~\ref{sec:analysis}.
% Figure generation tip:
% 1. execute <code_clustering>/plot_timeline.m
% 2. figures can be found in <figures>profile_timeline/

\vspace{-0.1cm}
\subsubsection{\textbf{Convergence of the estimated mutual information}}
%Our Detection Engine is based on the idea of calculating the mutual information. Although mutual information is agnostic to inference algorithms used by the \spyware, some challenges need to be carefully addressed. %as follows. \vspace{1mm}~\\
%\textbf{- Convergence of mutual information estimates:}
 An important aspect that is related to the use of mutual information  is the convergence of estimated mutual information to the actual mutual information from the data samples accessed by \sysname. That is, it is well known that calculating an estimate of mutual information with enough precision requires the access to multiple samples from both context and triggered actions\footnote{An estimate of the mutual information converges to actual mutual information asymptotically.}. Hence, one can argue that a malicious spyware---who is aware of the existence of \sysname as per assumption T4 in our threat model---may be tempted to reduce the frequency for which it monitors the actions with the goal of decreasing the number of samples used to estimate his mutual information and hence \emph{deceives} \sysname by reducing the associated \emph{suspicion score}\footnote{On average the actual mutual information is the upper bound for the estimate mutual information.}. 
To avoid such situation, we associate mutual information to actions instead of apps. That is, whenever an action takes place, we update the amount of mutual information between this particular action and all the context associated with it.  At any time point, once an app monitors this action, we copy the mutual information associated with this action to the app. Therefore, regardless of how frequent an app monitors actions, we associate to it the mutual information based on all samples in history---recall that the number of these samples are not controlled by the malicious app---not only on those to which it has access.%~\\

\vspace{-0.1cm}
\subsection{\sysname Mitigation Engine}\label{sec:mitigationimpl}
%The implementation of \sysname mitigation engine takes place as part of the main thread of the API call. 
When an application makes a call to one of the getter APIs, the mitigation engine checks if the calling application has an entry in the applications suspicion scores table. %(this table is constructed in the Detection Engine as shown in Figure~\ref{fig:detectengine}).
Afterward, the Mitigation Engine checks which \emph{Protection List} this API call is part of to know the corresponding suspicion score.
As mentioned in Section~\ref{sec:mitigation}, \sysname does not presume any mitigation treatment outperforms the others, and opportunistically selects a method and see the effect and gradually increases the mitigation. %The Mitigation Engine keeps monitoring the suspicion scores of all \spyware.
 If the suspicion score cannot be effectively decreased, \sysname will switch to another mitigation method. 
%The mitigation technique is then chosen according to the suspicious score. We first start with the row-masking with low probability and then increase the probability of masking and monitor how the mutual information decreases through the execution of the suspicious app and then the mitigation engine can decide to switch to the another mitigation technique if the masking technique doesn't decrease the mutual information. In Section~\ref{sec:evalmitigation}, we will show an evaluation of the effect of the different mitigation techniques on the degradation of mutual information and the performance of \spyware. 
To optimize the run-time of mitigation engine, we cache the decisions taken by the mitigation engine on this API call for each calling application while a separate thread update this cache based on mutual information values. The overhead on the API call is shown in Section~\ref{sec:analysis}.









==> mitigation.tex <==
\section{Mitigation}\label{sec:mitigation}
The mitigation module is the third module in \sysname which %is located in the \sysname service layer (as shown in Figure~\ref{fig:archdetect}) and it 
%handles three types of scenarios to deal with a possibly \spyware application. \sysname 

\r{Bo: please double check, but I think up to now we didn't say suspicion score is actually MI}
seeks a general way to hinder the \r{performance (is there a rather negative or neutral term to substitute?)} of \spyware to reveal user context without assuming which inference algorithm is used by a \spyware.
There are two solution regimes to achieve this: 1) imposing delays so that a \spyware cannot get the latest update in real time, and 2) tearing down the correlation between the actions monitored by \spyware and the context associated with them quantified by \emph{mutual information}. We call the mitigation method in the first regime \emph{delay}, and introduce three different mitigation methods in the second regime: \emph{suppression}, \emph{row-masking}, and \emph{feature-masking}.

\sysname keeps monitoring \emph{suspicion scores} of all apps. Once an app has suspicion score higher than a predefined value, the mitigation module is activated in order to reduce the suspicion scores of this app.
In order to achieve this goal, the mitigation module chooses one or more mitigation methods to apply to this app with a selected magnitude.
As a consequence, this suspicious app will receive obscured values.
The details of the proposed mitigation algorithms are discussed in the reminder of this section.
%The four mitigation methods are delay, noise imposing, falsification, and suppression as explained in Sections~\ref{sec:delay}, \ref{sec:suppression}, and \ref{sec:falsification} respectively. The three scenarios have a main objective which is reducing the correlation between the effect of monitoring the actions APIs in a monitor list and the context associated with it. Since \sysname is agnostic to which machine learning kernel \spyware is using, we need to find a general way to hinder the performance of \spyware even without knowing which kernel it is using. This is achieved by trying to reduce the mutual information that the application can see between the context and the values returned from the actions APIs.  

\subsection{Mitigate by Delay}\label{sec:delay}
Assume that a \spyware keep polling changes in actions in order to detect when certain adaptations take place. As shown in Section~\ref{sec:sca}, monitoring the time of the day with the changes done by context-aware app can reveal user's schedule. Hence, \sysname \emph{delays} all getters returning the values of actions so that a \spyware gets obscured and cannot get the up-to-date context.

If our system decides to use mitigation of delay, \sysname will choose a delay of $d$ minutes which is selected randomly.
To prevent a \spyware reveals which $d$ our system chooses, \sysname keeps a history of $d$ minutes of all monitored actions so that getters are kept to be unblocking calls.
As a consequence, a \spyware can still reconstruct user context sequences but with unknown offset. \sysname increases the delay adaptively based on how suspicious a \spyware is.

%which is a when an application is flagged with the \emph{delay} flag,  and it calls the API to return the value of ringer mode and the alarm volume, then these values will be retuned to the callee delayed by random delay so that, the ringer mode will be associated to time x and alarm volume will be associated to time y. \\
%\b{The delay ranges from ... to ... }

%\subsection{Mitigate by adding noise}\label{sec:noise}
%If an application is flagged by the \emph{noise flag}, a wrong setting value is reported upon request by imposing a gaussian noise. In this mitigation method, a noise magnitude is selected by \sysname and is defined as the variance of a gaussian distribution. The intuition behind is that since ConMan cannot get the precise values, it is harder to reveal protected contexts.

%then a wrong value for the requested setting will be reported. The intuition behind this scenario is not to fake the learnt profile knowledge like the previous technique, but to avoid learning any profiles at all. This is achieved by always reporting different values that the correct value. \\
%For example, if the current alarm volume has a high value, then the reported value is low. The falsified reported values are chosen from the acceptable ranges of each setting. For example, the alarm volume ranges from $1$ to $7$ and the music volume ranges from $1$ to $15$ so the values reported for the alarm volume lie between $1$ and $7$ and between $1$ and $15$ for the music volume. 

%\subsection{Mitigate by falsification}\label{sec:falsification}
%\b{here I should say that I flip a coin and when I change the variance and mean of the distribution of the value the mutual information change --$\rightarrow$ table}
%Similar to the previous mitigation method, falsification changes the settings individually upon being queried, but with a certain probability, which is the parameter of this policy. When \sysname decides to change one setting, it returns a value anywhere between possible minimum and maximum. Together with noise imposing method, both prevent ConMan to directly reveal user contexts.

%If an application is flagged by the \emph{falsify} flag, then a wrong value for the requested setting will be reported. The intuition behind this scenario is not to fake the learnt profile knowledge like the previous technique, but to avoid learning any profiles at all. This is achieved by always reporting different values that the correct value. \\
%For example, if the current alarm volume has a high value, then the reported value is low. The falsified reported values are chosen from the acceptable ranges of each setting. For example, the alarm volume ranges from $1$ to $7$ and the music volume ranges from $1$ to $15$ so the values reported for the alarm volume lie between $1$ and $7$ and between $1$ and $15$ for the music volume. 


\subsection{Mitigate by Suppression}\label{sec:suppression}
With the previous mitigation method, even though malicious software may not be able to get real-time update from delay mitigation, a \spyware can retrofit users' daily routing by aligning with a \emph{priori} knowledge, for example, the time a person usually goes to school or work. Once the personal schedule is derived, this mitigation will have no effect in the future.

The fundamental reason is that simply imposing a fixed delay will not reduce mutual information. Suppression mitigation, on the other hand, is designed to decrease the information a \spyware can harvest. The main idea of this mitigation technique is to give \spyware false adaptation actions by returning actions' values associated with other context. This is done by using the table of recent records maintained by \emph{Adaptation Records} (explained in Section~\ref{sec:trackapp}). When a \spyware is detected and suppression mitigation is chosen to be applied, \sysname mitigation module will randomly choose one in the latest $k$ records and report the action values of this record. The number $k$, herein, is the mitigation magnitude of this method.
%Hence, when a \spyware will reads the action values, it will read the values associated with other context. 
%In this mitigation, \sysname maintains a table with fixed number of rows to remembers the latest actions' changes. The number of rows is decided by our system and serves as a knob of mitigation magnitude, the more number of rows, the more effective this mitigation method is. Upon a new adaption is made, \sysname adjust the table accordingly and make an pointer randomly chooses one row in the table. Whenever a \spyware makes a setting query, \sysname returns the setting values of pointed row. 

\subsection{Mitigate by Masking}\label{sec:mitigation_mask}
Yet another mitigation to reduce mutual information is done by masking action values, i.e., returning zeros. We further explore two variants of the masking approach: \emph{row-masking} and \emph{feature-masking}. In the former approach, our system returns correct action values, but with a certain probability $p$, the system simply returns 0 to 
\spyware after context changes. The effect takes in place until the next adaption is made. The consequence is that a \spyware cannot infer anything during the masked periods, but can still make inferences based on the rest of the unmasked observations.
The feature-masking approach, in contrast, considers each action value individually. Upon one adaptation is made, each action has a certain probability to be masked. As a result, at any given time, a \spyware can only observe partial action values of an adaptation record, thus user context is less likely to be revealed. 

The decision of masking a row (in the former approach) or which action values to be masked (in the later approach) depends on flipping a biased coin with a selected probability $p$, which serves as the parameter of mitigation effectiveness.

\subsection{Mitigation Selection} \label{sec:mitigation_selection}
As we've justified before, two regimes of mitigation methods achieve different goals and can complement each other. In practical scenarios, we combine both delay mitigation with one in the second regime which reduces the mutual information. \sysname doesn't assume any mitigation can outperform another. In fact, a mitigation technique may be the most effective under a certain situation. Hence, \sysname logs the returned action values by the selected mitigation technique and calculates the mutual information between the true context values and the obfuscated action values. \sysname examines the effect of the imposed mitigation technique; if a \spyware can still survive under current mitigation treatment, i.e., the suspicion score still exceeds a predefined threshold, \sysname increases the mitigation magnitude first, and eventually switches to a different method.

%\subsection{Mitigation effect on context-aware application}
\subsection{Scope of mitigations}
\v{The mitigation is done in a per-app basis instead of a system-wide configuration. Hence, when mitigation is applied to a possibly \spyware, other well-behaved apps will still receive correct action values, including the context-aware adaptation app (i.e., the victim app). Therefore, mitigations cause no negative impact to context-aware apps.}



==> registry.tex <==
\section{Registry file}\label{sec:registery} 

%\begin{figure}[!t]
%\centering
%\lstset{language=XML, morekeywords={adapt,action,context}}
%\parbox{.98\linewidth}{\lstinputlisting{figures/registry_file_template}}
%\caption{Template of \sysname registry file.% showing how polymorphic methods are associated through \texttt{tags} and differentiated through ranges of operation under different contexts.  
% \label{fig:registrytemplate}}
%\end{figure}


%\begin{figure}[h]
%\centering
%  \lstset{language=XML, morekeywords={adapt,action,context}}
%{\lstinputlisting{figures/registry_file}}
%  \caption{Snippet of a \sysname registry file.}\label{fig:registry_example}
%\end{figure}
As mentioned in Section ~\ref{sec:sysarch}, the target of this paper is not to analyze the context-aware application code to extract the action-context relations. Hence, we use a simple way to get this relation from the developer who understands the semantics of his code. The developer provides a registry file with the context-aware application. The format of the the registry file is a simple XML file specified by the application developer. Broadly speaking, a developer has to specify the \emph{contexts} that are monitored by the context-aware application as well as the \emph{actions} triggered by this application. The process of generating the registry file can be automated by source code analyzers such as lint~\cite{androidlint}, or by analyzing the call flow graph of the decompiled android application using tools like SAAF~\cite{hoffmann2013slicing}.
%To fit in the Android flow, registry file is stored as an asset file packed with the application package file (APK).

During installation of new applications, \sysname checks the existence of the registry file. %inside the application package 
%APK.
 If exists, \sysname considers the associated application as a context-aware app and will apply its detection and mitigation mechanisms to protect this app from potential context exposures against any other suspicious apps.  In this section, we describe the structure of this XML file along with the post-processing steps performed by \sysname over this file.

%\r{Some adaptive context-aware application use third-party libraries. Hence the registry file is not straight forward for these applications. Indeed this registry file can be generated by static analysis tools to help the developer identify the actions and corresponding context~\cite{}}  \b{ - cite some papers that can generate the APIs call stack to help the developer or can be modified to generate a registry file}

\subsection{Registry file structure}
A context-aware application typically invokes a set of getter APIs in order to get the latest \emph{contexts} as well as a set of setter API to specify the corresponding \emph{actions}. Dependent on the application, different actions can be adapted based on different sets of contexts. Therefore, developers can specify several \texttt{adaptation} elements in a registry file in order to specify context and action correspondences. Thus, each adaptation should contain exactly one \texttt{context} and one \texttt{action} tag, both include one or more methods which are going to be used in the Java codes.

%For a context-aware application to monitor a context, it needs to invoke a call to a getter API in one of the Android Framework managers. For example, an application that triggers actions based on the battery capacity of the phone needs to call the \texttt{getBatteryCapacity()} API in the Android \texttt{BatteryManager}. Similarly, for a context-aware application to trigger an action, the application invoke a call to a setter API  in one of the Android framework managers (e.g. \texttt{setRingerMode()} in the Andorid \texttt{Audio Manager}). Therefore, to register the \emph{contexts} andthe  \emph{actions} of each context-aware application, it is enough to register the framework managers APIs used to monitor the contexts as well as the framework managers APIs used to trigger actions. 

Figure~\ref{fig:registry_example_2} demonstrates an example of the registry file. In this exemplar registry file, there are two adaptation policies. The first adaptation is relatively straightforward, which make decisions based on GPS location and update ringer mode and alarm volume accordingly.  In the second adaptation, the application adjusts the camera settings to accommodate, battery capacity, GPS location and transportation modality. Note that both actions have to be embedded in two different adaption policies although these two actions are conducted (partially) based on GPS location context because the decisions (i.e., actions) are computed independently. 

%\r{Bo's comment: I'm not sure we discussed this before, but in the Fig 3 the xml part, where are the functions defined? Since there is no getGPSlocation() method in Android. Do you raise another level of abstraction or are they pseudo methods? Maybe we need to clarify this a bit.}

%\r{Bo's 2nd comment: sorry I should raise this comment earlier but it just came to my mind: Again the xml part, what's the advantage to have developers specify separate different adaptions? I mean a developer can technically specify a super adaptation tag including every context and actions, which doesn't violate anything of file registry usage. What I can think of is that when user tends to decompose their logic and specify into several adaptation tags, the computation load of our system will not be that heavy. Should we cover this concern?}

%As shown in Figure~\ref{fig:registrytemplate}, the registry file is structured as a set of \emph{adaptations} where each \emph{adaptations} associates \emph{one} setter API (used to apply certain action) to the getter APIs used to monitor the contexts that triggers this specific action. Since the same context may be used to trigger more than one action, the registry file allows for multiple contexts to be repeated across different \emph{adaptations} and hence associated to different actions. Moreover, and to allow for complex behaviors, the register file captures the case where an action can be triggered based on different values from different contexts.


%For example, The application may perform an adaptation by calling \emph{$action_{1}$}, \emph{$action_{2}$}, ..., and \emph{$action_{n}$} at \emph{$context_{1}$}, \emph{$context_{2}$}, ..., and \emph{$context_{m}$}. %Hence the XML file will have the following format as shown in Figure~\ref{fig:registrytemplate}.\\ 
%\b{write here the set of actions we support like AudioManager, ContentObserver, WiFiManager, ConnectivityManager, CameraManager, ....}

%\subsubsection{Example}
%To illustrate the construction of the registry file, we provide a simple example in Figure~\ref{fig:registry_example}. In this example, we have three adaptation behaviors for adjusting two phone settings and one camera parameters under different contexts. The first two context-based adaptations are to change the ringer mode and the alarm volume based on the GPS location (similar to the motivating example in Section~\ref{sec:conman}). In the second adaptation, the application adjusts the camera settings to accommodate the user activity as well as the battery capacity. 
%Hence, the set of actions taken in this case are setting the focus mode, the quality of the picture saved, and the scene mode.





\begin{figure}[!t]
\centering
  \lstset{language=XML, morekeywords={adaptation,action,context}}
{\lstinputlisting{figures/registry_file}}
  \caption{Snippet of a \sysname registry file \vspace{-7mm}.}\label{fig:registry_example_2}
\end{figure}


%Hence, the \emph{action} list is the actual APIs called by the context-aware application to make the adaptation and the \emph{context} is the APIs called to know the current context.

%\begin{figure}[!h]
%\centering
%\lstset{language=XML, morekeywords={adapt,action,context}}
%\parbox{.98\linewidth}{\lstinputlisting{figures/registry_file}}
%\caption{Snippet of a \sysname registry file.% showing how polymorphic methods are associated through \texttt{tags} and differentiated through ranges of operation under different contexts.  
% \label{fig:registry_example}}
%\end{figure}
%\begin{figure}[!h]
%\centering
%\includegraphics[]{tikzfigures/monitorlist}
%\caption{Monitor lists created from registry file in Figure~\ref{fig:registry_example}.% showing how polymorphic methods are associated through \texttt{tags} and differentiated through ranges of operation under different contexts.  
% \label{fig:monitorlist}}
%\end{figure}


\subsection{Registry file processing}\label{sec:registryprocess}
Whenever a new application is installed, \sysname checks the existence of a registry file. Once \sysname finds a registry file,  several post-processing steps take place during the installation time of the application. In particular, \sysname parses the XML file  and the extracted information is then used to fill the following data structures:~\\
 %Figure~\ref{??} shows how \sysname flow extends the normal Android installation flow. This flow diagram shows the steps needed to post-process the registry file. 
 %
%There are two main data structures representing this module:
%\begin{enumerate}
\textbf{- Adaptation Records}: The purpose of this data structure is to keep track of actions taken by authentic context-aware apps and the context-change that triggered such action. This data structure takes the form of a map that records the values of the triggered actions, the set of the triggering contexts along with the timestamp for which this action was taken. The relation between contexts and actions are captured from the information described in the registry file.~\\~\\
\textbf{- Protection Lists}: 
In this data structure, we hold a list of all APIs that can be used by a ~\spyware to monitor the actions that are triggered by authentic context-aware apps.
%
%We need to detect malicious applications that are monitoring the changes in adaptations to infer the context as explained by the proposed ~\spyware in Section~\ref{sec:spycon}. Hence, a list of the functions that can be used by ~\spyware to read the current values of actions is needed. For every set of actions in each adaptation tag in the \emph{Registry File}, a list holding the corresponding functions that can read the action values is constructed. 
%
For the registry file example in Figure~\ref{fig:registry_example_2}, two lists are constructed for the two adaptation tags. The first Monitor List includes two functions, e.g., \texttt{getRingerMode} and \texttt{getAlarmVolume}. Similarly, the second list contains three functions.
 %\end{enumerate}
 
Parsing of the registry file, discovery of sets of actions, and creation of the data structures are implemented as part of \sysname context-adaptation registration module as shown in Figure ~\ref{fig:archdetect}. More details about the specific implementation of this module in the Android platform are shown in the implementation details Section~\ref{sec:implementation}.  %and with monitoring lists are implemented in \sysname service layer as described in the remainder of this section. 
 

 %\begin{figure}[!ht]
%  \centering
%    \includegraphics[width=\columnwidth, trim={3cm 3cm  2cm 1cm}]{figures/monitorlist}
 %    \caption{Monitor lists created from an example of registry file}
 %    \label{fig:monitorlist}
%\end{figure}
%
%\subsection{Effect of weight}
%\b{talk here on how the developer can provide the weights or we can train the weights ourselves}









